Efficient Deep Learning Pipelines for Accurate Cost Estimations Over Large Scale Query Workload

The use of deep learning models for forecasting the resource consumption patterns of SQL queries have recently been a popular area of study. With many companies using cloud platforms to power their data lakes for large scale analytic demands, these models form a critical part of the pipeline in managing cloud resource provisioning. While these models have demonstrated promising accuracy, training them over large scale industry workloads are expensive. Space inefficiencies of encoding techniques over large numbers of queries and excessive padding used to enforce shape consistency across diverse query plans implies 1) longer model training time and 2) the need for expensive, scaled up infrastructure to support batched training. In turn, we developed Prestroid, a tree convolution based data science pipeline that accurately predicts resource consumption patterns of query traces, but at a much lower cost. We evaluated our pipeline over 19K Presto OLAP queries from Grab, on a data lake of more than 20PB of data. Experimental results imply that our pipeline outperforms benchmarks on predictive accuracy, contributing to more precise resource prediction for large-scale workloads, yet also reduces per-batch memory footprint by 13.5x and per-epoch training time by 3.45x. We demonstrate direct cost savings of up to 13.2x for large batched model training over Microsoft Azure VMs.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> content/related.tex <==
\subsection{Black box inference}
Machine learning models are regarded as black boxes since users are concerned only with the input and output to the model. Earlier models explored simpler techniques such as KCCA \cite{ganapathi2009predicting}, for sub-space mapping of queries-resources, or standard regression analysis \cite{popescu2012same}. Recent years have witnessed the shift towards deep learning models such as feed forward network \cite{kipf2018learned,ortiz2018learning}, Tree CNN \cite{marcus2019neo}, RNN based networks \cite{ortiz2019empirical,sun2019end} or reinforcement learning \cite{marcus2020bao,marcus2019towards}. These models were designed to capture the inherent complexities of OLAP queries to which simpler models failed to do so. 

\subsection{White box inference}
Analytical models \cite{sen2018characterizing,wu2013predicting,rajan2016perforator,huang2017top} approach the problem differently than their machine learning counterparts. They attempt to shed light on the internal mechanisms of a database by modelling various aspects, such as data access and workload scheduling. Such models have been developed extensively for transactional based systems such as MySQL and Postgres or distributed data processing engines such as Hive and Hadoop. However, such models are highly specific to single databases and may be hard to develop.

==> content/results.tex <==
% Section deprecated. Please see section experiment_results.
% \begin{table*}[h]
%     \begin{subtable}[h]{0.45\textwidth}
%         \centering
%         \begin{tabular}{||c c c c c||}
%         \hline
%         \multicolumn{1}{||c}{} & \multicolumn{4}{c||}{K} \\
%         \multicolumn{1}{||c}{$P_f$} & 1 & 5 & 9 & 21 \\
%         \hline \hline
%         1 & 105.364 & 61.864 & 58.809 & 56.811 \\
%         100 & 91.739 & 55.687 & 51.048 & 50.313 \\
%         200 & 90.891 & 49.002 & 48.373 & 48.123\footnote{Although MSE score was lowest globally, model had poor epoch runtime and was not chosen as optimal} \\
%         300 & 91.073 & 50.955 & \textbf{48.218} & 48.782 \\
%         \hline \hline
%         \multicolumn{1}{||c}{CDF} & 0.357 &0.790 & 0.838 &	0.902 \\
%         \hline
%       \end{tabular}
%       \caption{N = 15}
%       \label{tab:sub_tree_node_lim_15}
%     \end{subtable}
%     \hfill
%     \begin{subtable}[h]{0.45\textwidth}
%         \centering
%         \begin{tabular}{||c c c c c||}
%         \hline
%         \multicolumn{1}{||c}{} & \multicolumn{4}{c||}{K} \\
%         \multicolumn{1}{||c}{$P_f$} & 1 & 5 & 11 & 20 \\
%         \hline \hline
%         1 & 60.595 & 56.935 & 57.570 & 57.465 \\
%         100 & 53.045 & 49.196 & 49.461 & 49.828 \\
%         200 & 52.366 & 50.708 & \textbf{47.785} & 48.957 \\
%         300 & 51.650 & 49.603 & 50.318 & 51.206 \\
%         \hline \hline
%         \multicolumn{1}{||c}{CDF} & 0.802 & 0.859 &	0.902 & 	0.924 \\
%         \hline
%       \end{tabular}
%       \caption{N = 32}
%       \label{tab:sub_tree_node_lim_32}
%      \end{subtable}
%      \hfill
%     \begin{subtable}[h]{0.85\textwidth}
%         \centering
%         \begin{tabular}{||c c c c c c c c||}
%         \hline
%         Median & Mean & SVR & Kipf & Full-1 & Full-100 & Full-200 & Full-300 \\
%         \hline \hline
%         169.191 & 140.170 & 106.156 & 63.577 & 54.207 & 50.089 & 52.734 & 50.698 \\
%         \hline
%       \end{tabular}
%       \caption{Benchmark performances}
%       \label{tab:benchmarks}
%      \end{subtable}
%      \caption{(a) \& (b) Recorded MSE errors ($min^2$) for models with various sub-tree node limit. $P_f$ represents the number of features chosen from our predicate Word2Vec model. Best performing models are in bold.  CDF value denoting the number of queries with minimally K sub-trees were displayed. Results were contrasted with benchmark performances in (c).}
%      \label{tab:mse_results}
% \end{table*}

% We present performance comparisons between our sub-tree models and selected benchmarks in Table \ref{tab:mse_results}. Our sub-tree CNN models were trained over 150 epochs for 3 rounds. In each round, the best performing iteration was used to compute the average MSE error for that model.

% \subsection{Capturing plan order sensitivity}
% We evaluated model performances over 150 epochs using Azure’s NC12s\_V3 cluster with single GPU restriction.
% Our experimental results indicate that Tree CNN models generally fared better than simpler SVR and feed forward models.

% \textbf{Information loss} - SVR and feed forward models were trained over an aggregation of features from both query and logical plans. In turn, this caused valuable plan order information to be lost. Tree CNN models were able to leverage these signals through the use of triangular kernels that were tuned to detect spatial patterns between a parent and its children. 

% \textbf{Variability of query plans} - For most OLAP engines, execution plans may change at the discretion of the optimizer. Presto's cost based optimizer utilizes real time cluster and table statistics to perform plan re-ordering to reduce projected cost of execution. This means that the same query, when executed under different settings or data, may yield a different plan! 

% Our Tree CNN pipelines work with dynamically inferred plans. Running the EXPLAIN command for Presto is a cheap operation which only takes seconds to complete and does not bottleneck model deployment. Yet, such on-the-fly inference of plans offers conveniences to users by abstracting away their concern for plan variability. This may be valuable to large companies such as MTX, where query plans may differ as underlying data is constantly changing across time.  

% \subsection{Hyper-parameter tuning} 
% We present 3 new parameters that may be tuned for performance. They are 1) $P_f$ $\rightarrow$ predicate features size, 2) K $\rightarrow$ query sub-trees selected and 3) N $\rightarrow$ max node count per sub-tree. 

% \textbf{Optimal configuration} - Experimental results in Table \ref{tab:mse_results} indicated that the (N-K-$P_f$) values for lowest MSE score were (15-21-200)\footnote{Although (15-21-200) contained a lower MSE score than (15-9-300), we regard the latter as the best performer for N = 15 due to better epoch runtime.} \& (32-11-200). Our results suggested that sampling of K sub-trees at 90th CDF percentile enables our model to perform better than full tree benchmarks. We reasoned that our sub-tree model had K times more features for inputs to the dense layer, unlike full tree models which collapses features across each node into a single vector via dynamic pooling. 

% \subsection{Optimizing hardware usage}
% We studied how our encoding and sub-sampling approach improves batch efficiency and training speeds. These improvements may translate to cost savings over cloud resources. 

% \textbf{Reduction in batch size} - The impact of 0-padding is significant given input size irregularities our benchmark models. For a given batch size of 32, our benchmark models consumed minimally 244MB of memory, which is 2.3x more than the largest sub-tree model at (32-20-300). Comparisons between sub-tree models (15-9-300) \& (32-11-200) relative to Full-300 yields a reduction of 12.9x and 5.5x respectively. 

% 0-padding was used to enforce dimensional consistency for inputs to all models. Padding for full tree models was based on the size of the largest tree present (1945 nodes). This meant padding a skewed distribution of small trees to the size of the largest. For the model proposed by Kipf, a large number of distinct predicates coupled with variations in table, join and predicate sets per query
% produced sparse and large input tensors. 

% \textbf{Reduction in training time} - Reductions in input data size consequently leads to faster training times owing to improved bandwidth utilization for data transfer between CPU to GPU and fewer computations needed over the data. Comparisons between sub-tree models (15-9-300) \& (32-11-200) relative to Full-300 yields speed up of 2.1x and 1.5x respectively.

% One interesting observation from Fig \ref{fig:hardware_consumption} is the disproportionate growth in epoch run time as we increase K. We attribute this to an inefficiency in our current code, which uses Tensorflow's \textit{tf\_map} operator to perform sequential convolutions over each sub-tree. This limitation may be addressed in future work. 

% \begin{figure*}[htp]
%     \centering
%     \begin{tabular}{@{}c@{}}
%         \includegraphics[scale=0.3]{pic/epoch_runtime.png}
%     \end{tabular}
    
%     \begin{tabular}{@{}c@{}}
%         \includegraphics[scale=0.3]{pic/batch_size.png}
%     \end{tabular}
    
%     \caption{Top: Comparison of average epoch time (min) for various models. Bottom: Comparison of average batch size (MB) of 32 rows for various models. (N-K-$P_f$) refers to the combination of maximum nodes per sub-tree - number of sub-sample trees - predicate feature size}
%     \label{fig:hardware_consumption}
% \end{figure*}

% \subsection{Cost savings}
% \begin{figure}[htb]
%     \includegraphics[scale=0.15]{pic/azure_cost.png}
%     \caption{Lower bound of costs using Azure NC\_V3 series clusters for model training at 150 epochs with varying batch sizes. Sub-15* \& sub-32* denotes best performing sub-tree model at N = 15 \& 32 respectively}
%     \label{fig:azure_cost}
% \end{figure}

% We evaluated the cost of model training over 150 epochs using Azure's NC6s\_V3 / NC12s\_V3 / NC24s\_V3 clusters. We chose the lowest possible cost among all clusters that permitted training with a specified batch size. Each cluster contained 1 / 2 / 4 Tesla V100 GPUs respectively and were priced at an hourly rate\footnote{Rates were up-to-date as of the time of writing and may change in future} of \$4.23 / 8.47 / 18.63. In multi-GPU clusters, data parallelism \cite{krizhevsky2014one} was employed to distribute batch workloads. We compared sub-tree models (15-9-300) \& (32-11-200), which were the best overall performers, against Full-100 \& Full-300. 

% \textbf{Scale-up penalties} - We observed diminishing returns in scaling up clusters of single GPU to multi-GPU instances. Fig \ref{fig:azure_epoch} showed that speed ups of at most 3x were observed in scaling from 1 to 4 GPUs. We attribute this to the communication overheads involved in synchronizing model training across multiple GPUs. This reason, coupled with a non-linear increase in pricing for NC24s\_V3 clusters, causes overall cost for multi-GPU training to be higher than single GPU instance.  

% \textbf{Batch size costs} - Fig \ref{fig:azure_cost} suggests that our sub-tree models were economically cheaper to train across a range of batch sizes as they were faster and had lower memory footprint. For large batches, Full tree models had to be trained on multi-GPUs due to out of memory errors, while sub-tree models could still be trained on a single GPU which was cost efficient. To quantify the impact of our sub-sampling approach, we observed training cost decline of \$217.12 to \$20.68 in switching from Full-300 model to (15-9-300) sub-tree model for a batch size of 256.

% \begin{figure}[htb]
%     \includegraphics[scale=0.2]{pic/azure_epoch.png}
%     \caption{Profiling of batch size against epoch runtime (min) for sub-tree model (15-9-300)}
%     \label{fig:azure_epoch}
% \end{figure}



==> versions/abstract_1.tex <==
We propose solutions that enable deep learning tree convolution models to be effectively applied over large data sets of query plans, for the purpose of forecasting the resource consumption of queries prior to execution. Our work surfaces two main problems in the course of training deep learning models over a large and diverse query plan set taken from the industry: 1) Large volumes of unique predicates renders existing query encoding techniques inefficient and 2) enforcing input shape consistency for a variety of large and small query plans causes redundant 0-padding which consumes scarce GPU memory and lengthens per-epoch training times. We propose a Word2Vec model trained over query vocabulary to derive a compressed embedding space for predicate tokens, thereby reducing query encoding space, and a novel sub-sampling algorithm to decompose large logical plans into smaller representations whilst preserving structural information needed for the tree convolution. Experimental results imply that our solution achieves better accuracy relative to existing full-tree convolution approaches, yet reduces input batch memory consumption by 12.9x and per-epoch training time by 2.1x. These improvements may be translated to direct cost savings over cloud infrastructures. 

==> versions/intro_1.tex <==
Present trends in big (OLAP) data query engines have evolved two ways; the shift towards execution over cloud-based infrastructure and the adoption of a decoupled compute-storage paradigm in their design. This is attributed to the rising adoption of the cloud as part of a company's technology stack. Cloud based platform-as-a-service have enticed firms to offload business data into managed data lakes at reasonable costs \cite{dageville2016snowflake} and offer localized compute resources for performing large query and aggregations over these data at low latency. 

While the decoupling of compute and storage has enabled such query engines to scale independently and elegantly across large volumes of data, query optimizers are no longer able to leverage on the inherent properties of the underlying data that enables them to make informed cost optimization decisions. On the engineering front, resource allocation for an incoming query becomes a challenge, as database administrators are unable to systematically forecast the anticipated resource a query is expected to consume simply via querying the optimizer. Cluster resource allocation thus becomes a trial-and-error process which could potentially lead to the deployment of sub-optimal policies; an under-allocation of resources could mean that a query will be starved of needed compute resources and miss its strict SLA deadlines, whilst an over-allocation of resources could mean unnecessary cost expenditure. In the context of large companies dealing with tens of thousands of incoming queries on a daily basis and managing query engines over massive clusters of machines, having a proper resource allocation framework is necessary to achieve substantial degree of cost savings within query SLA constraints \cite{gupta2008pqr,he2010comet}. 

\begin{figure}[htb]
    \includegraphics[width=\columnwidth]{pic/deployment_pipeline.pdf}
    \caption{Deployment pipeline for sub-tree CNN models}
    \label{fig:deployment_pipeline}
\end{figure}

To date, researchers have proposed both analytical models and deep learning models for the task of forecasting resource consumption of an unseen query. More details can be found in Section \ref{related-work}. We argue that the latter is more suitable in a highly dynamic industrial setup where multiple query engines are deployed to service different teams and where query engines may be deprecated early in favor of the new. In this case, the time invested in developing complex and engine specific analytical models do not justify the potential cost savings achievable.

Our work is an extension of the state-of-the-art tree convolution (Tree CNN) based models trained over the logical plan of queries. We argue that although such models are promising as they outperform \cite{marcus2019neo} modern database query optimizers on the task of forecasting a query's resource consumption pattern, they are not yet cost-efficient to be directly applied over the large and diverse query plans that are common in the industry.

\textbf{Research novelty} - In turn, we denote our contributions to the field below.

\begin{compactitem}[$\bullet$]
    \item We present a case study over SQL queries gathered from the industry to justify the need for a more cost-efficient approach in building Tree CNN pipelines. In particular, we emphasise the need for space-efficient encoding techniques that scale with an ever increasing corpus of query predicates and the need to reduce excessive 0-padding when training against inconsistent query plan sizes due to scarce GPU memory. 
    
    \item We present two solutions for the above mentioned problems. The first is a Word2Vec model trained over a corpus of predicates which reduces per-token embedding length and the second a sub-sampling algorithm for decomposition of large query plans in a manner that fully preserves breadth level information needed for Tree CNN. 
    
    \item We incorporated these solutions into our sub-tree CNN model and show that our model can achieve comparable accuracy with standard full tree CNN models at much lower training cost over Microsoft Azure infrastructures. 
\end{compactitem}

The remainder of this paper is as follows. In Section \ref{background}, we introduce the foundational concepts needed for training tree convolution networks over query plans. In Section \ref{case_study}, we present a case study over real data set from the industry to justify the value of our work. In Section \ref{solution}, we present the training procedure for encoding predicates using Word2Vec model and our sub-sampling algorithm implementation. We present our experimental results in Section \ref{experiment_results} before concluding in Section \ref{conclusion} and a review of related works in Section \ref{related-work}.

\subsection{Research inspiration}
Our work is heavily inspired by use cases from a large ride hailing company managing a data lake of more than 20 Petabytes in the cloud. In order to service the hundred of thousands of OLAP queries issued by internal teams, the company has resorted to managing multiple Presto clusters \cite{sethi2019presto} over cloud infrastructures. Monthly expenditure on such compute resources form a large portion of overall tech expenses. We shall use the abbreviation MTX to address this company for this review. 

Although our experiments were conducted using data specific to MTX, we believe that the general techniques can be distilled and applied to any other companies managing data lakes at similar scale. 

==> versions/intro_2.tex <==
Present trends in big (OLAP) data query engines have evolved two ways; the shift towards execution over cloud-based infrastructure and the adoption of a decoupled compute-storage paradigm in their design. This is attributed to the rising adoption of the cloud as part of a company's technology stack. Cloud based platform-as-a-service have enticed firms to offload data into managed data lakes at reasonable costs \cite{dageville2016snowflake} and offer pay-as-you-use compute resources for performing large queries over these data. This makes resource provisioning managing query engines a huge challenge and cost saving opportunity. In a decoupled compute-storage architecture, database administrators are unable to systematically forecast the anticipated resource a query is expected to consume without first executing it. This could lead to over-allocation of resources which incurs additional cost, or under-allocation of resources at the risk of a query missing SLA deadlines. In the context of large companies dealing with hundreds of thousands of incoming queries on a daily basis and managing query engines over massive clusters of machines, having a proper resource allocation framework is necessary to achieve substantial degree of cost savings within given SLA constraints \cite{gupta2008pqr,he2010comet}.

Our work is heavily inspired by use cases from a large ride hailing company managing a data lake of more than 20 Petabytes in the cloud. In order to service the hundred of thousands of OLAP queries issued by internal teams, the company has resorted to managing multiple Presto clusters \cite{sethi2019presto} over multi-cloud infrastructures. Monthly expenditures on cloud form a large portion of overall expenses, emphasising the need for a proper resource allocation framework. We shall use the abbreviation MTX to address this company. 

\begin{figure}[htb]
    \includegraphics[width=1\linewidth]{pic/deployment_pipeline.pdf}
    \caption{Deployment pipeline for sub-tree CNN models}
    \label{fig:deployment_pipeline}
\end{figure}

To date, researchers have proposed end-to-end deep learning pipelines to aid in forecasting the resource consumption of new queries. Such models may be integrated, as illustrated in Fig \ref{fig:deployment_pipeline}, to systematically guide resource controllers into provisioning the right amount of compute units needed to run the query. However, we argue that such methods are not yet cost-efficient to be directly applied over the set of queries at variety and volume. Present research do not explore efficient and practical encoding techniques needed to control the encoding length of query predicates, nor do they adequately address the issue of excessive padding used to reconcile different query plan sizes, which leads to a slow and GPU-memory intensive model training. These issues are elaborated in Section \ref{case_study} and causes model training over cloud to be unnecessarily expensive. 

Our work extends the state-of-the-art tree convolution (Tree CNN) based pipelines to improve their cost efficiencies. We introduce our sub-tree convolution (CNN) pipeline, which consists of a model trained using sampled sub-trees from a full query plan, and tree encoding techniques. Experimental results indicate that training based on our pipeline is consistently cheaper to over Azure clusters across a range of batch sizes.

\textbf{Research novelty} - We denote our contributions below.

\begin{compactitem}[$\bullet$]
    \item We present a case study over SQL queries gathered from MTX. Our study revealed the presence of a large number of distinct predicates and a wide disparity in query plan sizes. Thereafter, we show why present techniques are not space-efficient for predicate encoding and highlight the impact of excessive padding on scarce GPU memory.
    
    \item We present two solutions for the above mentioned problems. The first is a Word2Vec model trained over a corpus of predicates which reduces per-token embedding length and the second a sub-sampling algorithm for decomposition of large query plans in a manner that fully preserves breadth level information needed for tree convolution. 
    
    \item We incorporated these solutions into our sub-tree CNN pipeline and show that our models can achieve better accuracy with standard full tree convolution models at much lower training cost over Azure infrastructures. 
\end{compactitem}

The remainder of this paper is as follows. In Section \ref{background}, we introduce the foundational concepts needed for training tree convolution networks over query plans. In Section \ref{case_study}, we present a case study over real data set from the industry to justify the value of our work. In Section \ref{solution}, we present the training procedure for encoding predicates using Word2Vec model and our sub-sampling algorithm implementation. We present our experimental results in Section \ref{experiment_results} before a review of related works in Section \ref{related-work} and concluding in Section \ref{conclusion}.

